Log-DenseNet: How to Sparsify a DenseNet

Skip connections are increasingly utilized by deep neural networks to improve accuracy and cost-efficiency. In particular, the recent DenseNet is efficient in computation and parameters, and achieves state-of-the-art predictions by directly connecting each feature layer to all previous ones. However, DenseNet's extreme connectivity pattern may hinder its scalability to high depths, and in applications like fully convolutional networks, full DenseNet connections are prohibitively expensive. This work first experimentally shows that one key advantage of skip connections is to have short distances among feature layers during backpropagation. Specifically, using a fixed number of skip connections, the connection patterns with shorter backpropagation distance among layers have more accurate predictions. Following this insight, we propose a connection template, Log-DenseNet, which, in comparison to DenseNet, only slightly increases the backpropagation distances among layers from 1 to ($1 + \log_2 L$), but uses only $L\log_2 L$ total connections instead of $O(L^2)$. Hence, Log-DenseNets are easier than DenseNets to implement and to scale. We demonstrate the effectiveness of our design principle by showing better performance than DenseNets on tabula rasa semantic segmentation, and competitive results on visual recognition.

==> table_logdense.tex <==
(12,16) m=L
	& 29.30 & 24.27 & 13.63 &  7.23 & 62.48 & 56.85 & 42.97 & 29.14 & 12.99 &  5.66 &  3.80 &  2.03 \\
(12,16) m=N
	& 29.24 & 23.40 & 13.15 &  7.59 & 62.79 & 55.34 & 42.61 & 30.59 & 10.96 &  6.35 &  3.84 &  2.11 \\
(12,16) m=E
	& 29.26 & 21.82 & 13.11 &  7.45 & 61.17 & 53.73 & 41.92 & 30.72 & 12.53 &  5.51 &  3.83 &  2.27 \\
\hline
(12,24) m=L
	& 22.85 & 18.86 & 10.51 &  5.98 & 57.04 & 52.41 & 37.48 & 26.36 &  8.77 &  4.43 &  3.20 &  1.94 \\
(12,24) m=N
	& 25.22 & 19.74 & 10.53 &  6.46 & 56.70 & 51.35 & 37.42 & 26.96 &  8.32 &  4.61 &  3.32 &  2.10 \\
(12,24) m=E
	& 24.51 & 18.45 & 10.66 &  6.56 & 55.93 & 48.65 & 36.88 & 27.80 & 10.30 &  4.64 &  3.24 &  2.05 \\
\hline
(12,32) m=L
	& 20.39 & 13.92 &  9.11 &  5.48 & 53.64 & 48.63 & 34.42 & 24.21 &  7.68 &  4.07 &  2.93 &  1.85 \\
(12,32) m=N
	& 21.68 & 17.26 &  9.48 &  6.00 & 54.05 & 47.32 & 34.29 & 24.70 &  7.10 &  4.40 &  3.12 &  1.92 \\
(12,32) m=E
	& 22.24 & 16.31 &  9.32 &  6.15 & 52.43 & 44.46 & 33.40 & 25.57 &  7.72 &  4.34 &  3.08 &  1.90 \\
\hline
(32,16) m=L
	& 21.40 & 12.23 &  9.36 &  5.96 & 58.92 & 43.82 & 36.66 & 25.32 &  4.78 &  3.61 &  3.42 &  1.97 \\
(32,16) m=N
	& 24.81 & 12.95 &  9.11 &  6.45 & 60.61 & 48.12 & 38.20 & 27.48 &  5.41 &  3.57 &  3.10 &  1.94 \\
(32,16) m=E
	& 19.65 & 12.42 &  9.49 &  6.21 & 51.89 & 42.82 & 38.21 & 26.81 &  5.07 &  3.39 &  2.91 &  1.96 \\
\hline
(32,24) m=L
	& 15.46 &  9.91 &  8.20 &  5.03 & 51.13 & 37.46 & 32.75 & 22.73 &  3.87 &  3.20 &  3.18 &  1.77 \\
(32,24) m=N
	& 21.13 & 12.09 &  7.75 &  5.74 & 54.91 & 43.57 & 33.59 & 25.08 &  4.80 &  3.37 &  2.84 &  1.82 \\
(32,24) m=E
	& 14.80 &  9.76 &  7.75 &  5.43 & 45.42 & 36.92 & 32.74 & 24.80 &   -   &   -   &   -   &   -   \\
\hline
(32,32) m=L
	& 12.86 &  8.58 &  7.10 &  4.81 & 45.99 & 32.87 & 29.46 & 21.77 &  3.68 &  3.00 &  2.85 &  1.76 \\
(32,32) m=N
	& 19.18 & 11.04 &  7.47 &  5.65 & 52.41 & 38.18 & 30.30 & 23.79 &  4.07 &  3.06 &  2.66 &  1.82 \\
(32,32) m=E
	& 13.60 &  8.89 &  7.03 &  4.94 & 41.85 & 34.26 & 30.17 & 23.87 &  3.80 &  2.99 &  2.39 &  1.95 \\
\hline
(52,16) m=L
	& 15.16 & 11.77 &  8.30 &  5.13 & 50.09 & 42.70 & 33.83 & 23.45 &  3.78 &  3.62 &  2.30 &  1.66 \\
(52,16) m=N
	& 22.66 & 11.65 &  7.78 &  6.80 & 58.29 & 47.31 & 35.17 & 27.99 &  5.81 &  3.94 &  2.69 &  1.98 \\
(52,16) m=E
	& 15.91 & 10.85 &  8.16 &  6.09 & 46.29 & 38.96 & 35.00 & 26.58 &  3.93 &  3.12 &  2.54 &  1.85 \\
\hline
(52,24) m=L
	& 12.04 &  9.24 &  6.91 &  4.34 & 42.81 & 36.72 & 29.42 & 20.99 &  3.53 &  3.35 &  2.40 &  1.64 \\
(52,24) m=N
	& 24.18 & 11.60 &  6.92 &  5.83 & 53.92 & 42.65 & 31.97 & 26.07 &  4.96 &  3.72 &  2.59 &  1.90 \\
(52,24) m=E
	& 12.84 &  9.13 &  7.32 &  5.03 & 41.68 & 34.56 & 31.74 & 24.19 &  3.59 &  3.15 &  2.28 &  1.80 \\
\hline
(52,32) m=L
	& 10.76 &  8.20 &  6.34 &  4.56 & 40.76 & 34.27 & 28.16 & 20.58 &  3.30 &  3.08 &  2.25 &  1.72 \\
(52,32) m=N
	& 17.66 &  9.70 &  6.51 &  6.10 & 52.72 & 41.04 & 29.47 & 24.79 &  4.01 &  3.21 &  2.41 &  1.89 \\
(52,32) m=E
	& 11.44 &  8.18 &  6.53 &  4.98 & 38.85 & 32.12 & 29.42 & 23.10 &  3.23 &  2.92 &  2.22 &  1.78 \\
\hline

==> table_logdense_wrapper.tex <==
\begin{table}
\centering
\subfloat[Performance of three connection strategies on 27 different settings.]{
\resizebox{\textwidth}{!}{
\begin{tabular}{ c | c c c c | c c c c | c c c c}
    \hline
        & \multicolumn{4}{c|}{CIFAR10} 
        & \multicolumn{4}{c|}{CIFAR100} 
        & \multicolumn{4}{c}{SVHN}\\
                    &  1/4  &  1/2  &  3/4  & 1 
                    &  1/4  &  1/2  &  3/4  & 1 
                    &  1/4  &  1/2  &  3/4  & 1 \\
    \hline
\input{table_logdense.tex}
\hline
\end{tabular}}
}

\subfloat[Percentage of experiments \logdense V1(m=L) is outperformed]{
    \begin{tabular}{c|cccc}
    \hline
Method    & 1/4 & 1/2 & 3/4 & 1\\
    \hline
\input{table_dsm_compare_cnt.tex}
    \hline
    \end{tabular}
    
    \label{tab:dsm_cnt}
}
~
\subfloat[Relative percentage increase in error rate from \logdense V1(m=L) ]{
    \begin{tabular}{c|cccc}
    \hline
Method   & 1/4 & 1/2 & 3/4 & 1  \\
    \hline
\input{table_dsm_compare_diff.tex}
    \hline
    \end{tabular}
    \label{tab:dsm_gap}
}

\caption{\textbf{(a)} Each entry represents the top-1 error rate after 1/4, 1/2, 3/4, and 1 of the total FLOPS are computed on CIFAR10, 100, and SVHN. $(n,g)$ represents the number of feature layers in each of the three dense blocks. $m=L,N,E$ represents the connection strategies \logdense V1, \nearest, and \evenspace, each of which connects to $1+\log (i)$ layers at depth $i$, but the \logdense V1 has $O(\log(L))$ \pbd while the other two have $O(\frac{L}{\log L})$.\logdense V1 outperforms the others clearly. 
\textbf{(b)} Percentage of the 27 experiments that \logdense is outperformed by \nearest and \evenspace, at each cost location. Lower means \logdense is consistently better.
\textbf{(c)} The average over the 27 comparisons of the relative increase in error rate from those of \logdense by \nearest and \evenspace. Higher means \logdense is better with higher margin. 
}
\label{tab:table_dsm_full}
\end{table}

